Analysis of the flow of granular materials through a screw conveyor

Screw conveyors are widely employed in industry for the bulk transport of particulate materials. Several studies have attempted to correlate the discharge rate with the rotation speed of the screw via experiments and particle dynamics simulations. However, a detailed mechanical model that would assist in the optimal design of screw conveyors has not been attempted. In this study, we first construct a simple model that assumes the entire granular medium to move as a rigid body sliding along the surfaces of the screw and barrel. By enforcing the balances of linear and angular momentum to a suitably chosen continuum element, we show that under certain limiting conditions, the discharge rate for a given angular velocity and screw geometry can be obtained. Further, we show that the discharge can be maximized by setting the ratio of the pitch to barrel diameter to a particular value. We then study the detailed flow within the conveyor using the Discrete Element Method, which reveals that a significant fraction of the material exhibits solid body motion, in agreement with the simple model. We assess the effect of relaxing the limiting conditions employed in the model, thereby determining the connection between the friction at the walls and the kinematics of flow. Finally, the trend in variation of average axial velocity with the pitch to barrel diameter ratio in the presence of gravity is compared with that from our model and simulations in the absence of gravity. We observe that both the trends are qualitatively the same indicating that the dependence of average axial velocity on the geometry of the conveyor is not altered by the introduction of gravity.

==> sections/acknowledgements.tex <==
\textit{I am grateful to Prof Prabhu R Nott for the opportunity to carry out my research under his supervision. I really appreciate the support and the freedom to venture into whatever it was that I found captivating. I have equally enjoyed sitting through his lectures and doing research with him.}\\

\textit{I thank my labmate Ravi Gautam for his patient listening to my problems and for his constant encouragement. It was really nice to have him around in the lab. I have had a really good time  indulging in conversations with him on anything  and everything. I also thank Peter and krishnaraj for helping me in getting onboard with DEM simulations. The memories of my trip to IIT Bombay with Prachi, and to the APS-DFD conference with Phani will always be pleasant to recall.}\\

\textit{I thank the Gymkhana snooker club where I would recharge myself after a long tiring day in the lab. I am fortunate to be blessed with friends who made my stay here at IISc memorable. I am also going to miss those late night discussions with Raj on philosophy, psychology, theology and other important stuff that matter!}\\

\textit{I am indebted all my teachers starting from kindergarten who taught me how to conform and especially the ones who taught me when not to. I specially thank Mr Nabaraj Dhungana who has inspired me with the sincerity of his endeavors of helping students recognize their potential. I thank Prof. Raji George for his unwavering confidence in me at a time when I myself wasn't sure of where I was heading.} \\

\textit{I thank my cousin, Abhay Kumar, who has  acted as a mentor to me in my academic journey. I am blessed to have a friend like Umang who has been very encouraging all along. Finally, I thank my parents and my brother Manish for their unconditional love and support.} \\

\textit{In the pursuit of objective truth, which academic research symbolizes, it's not that difficult to lose yourself. But the beauty of it is, each time that happens, you come back stronger with a reinforcement of the reasons that led to that pursuit in the first place. It won't be an exaggeration if I say I have learned equally about myself as I have about the problem of my thesis. I am grateful to the sequence of events that have led me to having this experience.}

==> sections/introduction.tex <==
A screw conveyor is a device that consists of a helical screw blade mounted on a shaft which is placed concentrically inside a barrel. Screw conveyors were used in ancient Greece and Egypt to draw water for irrigation purposes or to drain water from low lying mining areas \citep{chakarborthy2014product}. Today screw conveyors in the irrigation sector have largely been replaced by motorized pumps. However they are extensively employed for powder and grain transportation in the pharmaceutical and food processing industries. Material to be conveyed is poured in from one end, which is carried by the virtue of the rotating blades to the outlet section.\\

Owing to its large industrial relevance, there have been several studies in the past that have tried to study solid flow rate as a function of rotational speed of the screw. Owen et. al. \cite{owen2009prediction} have attempted to study the effect on screw conveyor performance with its inclination with respect to the horizontal plane; and the volumetric fill level of the bulk material using DEM (Discrete Element Method), a particle based simulation technique. The dependence of flow rate on the magnitude of forces between cohesive grain partcles was investigated by Hou et. al. \cite{hou2014study}. Cleary \cite{cleary2007modelling} employed DEM to study the draw down
patterns in the hoppers and the effect of particle shape on these patterns. Screw conveyor with flexible discrete spiral blades was proposed by Tian et. al. \cite{tian2018research} to solve the problem of material gathering between the screw and the tube wall in the traditional screw conveyor. They also built a power consumption model for their proposed alternative design. The complex nature of flow inside a screw conveyor has resisted attempts to theoretically model the flow. However, an analysis of flow rate in a screw conveyor was attempted by Wu \cite{wu1978transport} by reducing it to a rectangular channel. In practical design, a rough
estimate of the performance is based on an empirical equation
from the database of practical machines.\citep{colijn1985mechanical,woodcockmason}. In this work, we aim to provide an insight into the dependence of flow rate predominantly on the geometry of the screw conveyor. We will be working with a horizontal screw conveyor where the rotation speed of the inner shaft is small enough to guarantee us being in the slow flow regime.\\

In the problem of calculating the flux of a liquid flowing through a pipe, the standard approach is to solve the conservation equations supplemented with a constitutive relationship by supplying the necessary initial and boundary conditions. Initially, an analytical solution is sought. In the absence of one, we resort to numerically solving the set of equations. The challenges associated with the general approach stated above, in the context of the problem at hand are as follows: the non-availability of a constitutive relation that is valid over the entire range of granular systems \citep{rao2008introduction}, and complexity of the geometry which renders an analytical solution impossible. However, if one chooses to march ahead with the existing continuum  models \citep{goddard1986dissipative,johnson1987frictional,johnson1990frictional,savage1998analyses,jop2006constitutive,nott2009classical} bearing the risk of failure to capture all the flow features, he has to employ numerical techniques which can, at times, be a daunting task.\\\\
A simplistic model proposed by Roberts \cite{roberts1999influence} to relate the flow rate through a screw conveyor to its rotation speed, replaces the complex geometry of the conveyor with a plunger as shown in Figure \ref{plunger}. The plunger consists of an annular disk which can slide on a shaft within the barrel, covering a distance equal to the pitch, $p$, of the screw in a time corresponding to the time period of rotation of the screw. As the disk slides, whatever material is trapped in the annular region is ejected out. The corresponding equation of number of particles ejected out per second, $n$, is as follows.\\
\begin{equation}
n=\nu \frac{\pi (D_b^2-D_s^2)}{4V_p}pN
\end{equation}\\
where $\nu$ is the solid fraction, $V_p$ is the average volume of a single grain, $N$ is the number of rotation of the screw per second, and $D_b$ and $D_s$ are the diameters of the barrel and the screw shaft respectively.\\
\begin{figure}[!htb]
	\centering
	\includegraphics[width=\linewidth]{introduction/plunger}
	\caption{A simplification to geometry proposed by Roberts \cite{roberts1999influence}, to relate the flow rate to the rotation speed of screw conveyor.}
	\label{plunger}
\end{figure}
\\
The current work aims to develop a model based purely on mechanics to relate the discharge to the rotation speed of screw, without compromising the intricacies of geometry. In section II, we assume the simplest case of helical channel being filled with a solid plug which slides along the flight surface and gets ejected out ultimately as a consequence of screw rotation. A differential element of the plug is suitably chosen on which the momentum balances are enforced in order to arrive at an expression for the rate of discharge. As will be seen, without knowledge of the stresses on the various surfaces, a solution of discharge is only admissible in the limiting case of friction vanishing on the screw surface. Despite this simplification, the model provides good insight into the mechanism of conveyance.\\\\
To obtain a general expression for discharge using our model, we need information about the stresses on the various surfaces. That's where we employ Discrete Element Simulations where we now impose a finite coefficient of friction on the screw and the barrel surfaces. We study the effect of introducing friction on the flow by analyzing the deviations from the solid plug solution, in section III. We also identify certain trends in the stress profiles as we move from one flight surface to the another along the axis of screw. In all of the work till this point, the effect of gravity is absent. This is because we want to isolate the effect on the flow, solely because of its geometry from that induced by gravity.\\\\ 
We also perform simulations on the conveyor in the presence of gravity,  results of which are presented in section III. The kinematics is not simple enough to allow for any general remarks. An interesting result however is that of the variation of average axial velocity with the ratio of pitch to barrel diameter. The variation is similar to that obtained from DEM simulations without gravity, and our model. These results also suggest a tentative range for the pitch to barrel diameter ratio for achieving maximum discharge.






































